Interpreting Face Inference Models using Hierarchical Network Dissection

This paper presents Hierarchical Network Dissection, a general pipeline to interpret the internal representation of face-centric inference models. Using a probabilistic formulation, our pipeline pairs units of the model with concepts in our "Face Dictionary", a collection of facial concepts with corresponding sample images. Our pipeline is inspired by Network Dissection, a popular interpretability model for object-centric and scene-centric models. However, our formulation allows to deal with two important challenges of face-centric models that Network Dissection cannot address: (1) spacial overlap of concepts: there are different facial concepts that simultaneously occur in the same region of the image, like "nose" (facial part) and "pointy nose" (facial attribute); and (2) global concepts: there are units with affinity to concepts that do not refer to specific locations of the face (e.g. apparent age). We use Hierarchical Network Dissection to dissect different face-centric inference models trained on widely-used facial datasets. The results show models trained for different tasks learned different internal representations. Furthermore, the interpretability results can reveal some biases in the training data and some interesting characteristics of the face-centric inference tasks. Finally, we conduct controlled experiments on biased data to showcase the potential of Hierarchical Network Dissection for bias discovery. The results illustrate how Hierarchical Network Dissection can be used to discover and quantify bias in the training data that is also encoded in the model.

==> algs.tex <==
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{algorithmic,algorithm2e,float}


\newcommand{\algIOU}{
\begin{algorithm}[h]
% \tiny %\small, \footnotesize, \scriptsize, or \tiny
\caption{IOU calculation for the   layer $\mathcal{L}$ in network $\mathcal{N}$}
\label{alg:IOU}
% \algsetup{linenosize=\tiny}
%   \scriptsize
% \algsetup{linenosize=\tiny}
%   \scriptsize
%   \begin{algorithmic}[1]
     No. of Images $\longrightarrow$ \(N\) \\
    \indent No. of Hidden Units $\longrightarrow$ \(M\) \\
    \indent No. of Concepts in Dictionary $\longrightarrow$ \(K\) \\
    \indent Activation Map Size $\longrightarrow$ \((H, W)\)
    \begin{enumerate}
        \item Take a forward pass across the dataset and store activation maps as \emph{A}.
    \end{enumerate}
    
    \indent Activation Maps (A) $\longrightarrow$ \((M, N)_{H \times W}\)
    \begin{enumerate}[resume]
        \item Calculate  threshold \emph{thr} as 0.995 quantile of all spatial locations for each unit.
    \end{enumerate}
    
    Tally Intersection (TI) $\longrightarrow$ \((M, K)\) \\
    \indent Tally Union (TU) $\longrightarrow$ \((M, K)\)
    \begin{enumerate}[resume]
        \item Initialize TI, TU = 0
        \item Tally IOU across the entire dictionary for each unit-concept pair \\
        for \(m = 1,..., M\):
        \begin{itemize}
            \item[] Unit threshold = \(t_{m}\)     \\
            for \(n = 1,..., N\):
            \begin{enumerate}
                \item feature map = \(A_{m, n}\)
                \item upsample \(A_{m, n}\) to original size \\
                if max(\(A_{m, n}\))\textgreater\(t_{m}\):
                \begin{enumerate}
                    \item threshold feature map (\textbf{\(A_{m, n}^{t}\)})
                    \item for \(k = 1,..., K\):
                    \begin{itemize}
                        \item[] concept mask = \(M_{k}\)
                        \item[] \(TI[m, k]\) += \((A_{m, n}^{t}\)$\cap$\(M_{k}\))
                        \item[] \(TU[m, k]\) += \((A_{m, n}^{t}\)$\cup$\(M_{k}\))
                    \end{itemize}
                \end{enumerate}
            \end{enumerate}
        \end{itemize}
        \item Return the IOU for each unit concept as the dataset wide sum of intersections over sum of unions \\
        \[IOU_{m,k} = \frac{TI[m, k]}{TU[m, k]}\]
    \end{enumerate}
%   \end{algorithmic}
\end{algorithm}

}


\newcommand{\algProbability}{
\begin{algorithm}
\caption{Probability estimation for clustered concepts.}
% \algsetup{linenosize=\tiny}
%   \scriptsize
%   \begin{algorithmic}[1]
    \noindent No. of Hidden Units $\longrightarrow$ \(M\) \\
    for \(m = 1,..., M\):
    \begin{enumerate}
        \item Identify the cluster for that unit based on concept with highest IOU.
    \end{enumerate}
    \indent \indent No. of Concepts in a Cluster $\longrightarrow$ \(K\)
    \begin{enumerate}[resume]
        \item Initialize Concept Scores (CS) for all K concepts \\
        for \(k = 1,..., K:\)
        \begin{itemize}
        \item[] \(CS_{k} = 0\)
    \end{itemize}
    \end{enumerate}
    \begin{enumerate}[resume]
        \item Obtain activation maps belonging to the cluster and sort them by their maximum activation score.
    \end{enumerate} 
    \indent \indent No. of Images belonging to a cluster $\longrightarrow$ \(N\) \\
    \indent No. of Images belonging to a single concept $\longrightarrow$ \(N_{k}\) \\
    \indent Chosen Maps (A) $\longrightarrow$ \((M, N)_{H \times W}\)
    \begin{enumerate}[resume]
        \item Normalize the range of scores for the maps of that cluster to [0,1] and then tally concept scores by also accounting for their rank in the cluster. \\
        for \(n = 1,..., N\):
        \begin{itemize}
            \item[] rank = \(n\) \\
            fmap\_score = max(\(A_{m, n}\)) \\
            for \(k = 1,..., K:\)
            \begin{itemize}
                \item[] if fmap belongs to concept \(k\):
                \begin{itemize}
                    \item[] \(CS_{k}\) += ($rank\times fmap\_score$)
                \end{itemize}
            \end{itemize}
        \end{itemize}
        \item Normalize the scores by the number of images that belong to each concept. \\
        for \(k = 1,..., K:\)
        \begin{itemize}
            \item[] \(CS_{k} = CS_{k} / N_{K}\)
        \end{itemize}
        \item Normalize the list of concept scores by the sum of the list to showcase their relative probabilities. \\
        for \(k = 1,..., K:\)
        \begin{itemize}
            \item[] \(CS_{k} = CS_{k} / sum(CS_{K})\)
        \end{itemize}
    \end{enumerate}
\label{alg:Probability}
\end{algorithm}
}
